Conway's doughnuts

Morley's Theorem about angle trisectors can be viewed as the statement that a certain diagram `exists', meaning that triangles of prescribed shapes meet in a prescribed pattern. This diagram is the case n=3 of a class of diagrams we call `Conway's doughnuts'. These diagrams can be proven to exist using John Smillie's holonomy method, recently championed by Eric Braude: `Guess the shapes; check the holonomy.' For n = 2, 3, 4 the existence of the doughnut happens to be easy to prove because the hole is absent or triangular.

==> dough_dot_bib <==
@article{conway:three,
author="John Conway",
title="Morley's trisector theorem",
journal="Math. Intelligencer",
year="2014",
volume="36",
pages="3"
}


@phdthesis{mohanty:thesis,
author       = {Yana Mohanty}, 
title={Hyperbolic polyhedra: volume and scissors congruence},
school       = {UCSD},
year         = {2002},
note={\url{http://math.ucsd.edu/~thesis/thesis/ymohanty/ymohanty.pdf}}
}

@misc{thurston:three,
author = "William P. Thurston",
title={Geometry and topology of three-manifolds},
year="1980",
note={Princeton University Math. Dept.}
}

@article {milnor:hyperbolic,
    AUTHOR = {Milnor, John},
     TITLE = {Hyperbolic geometry: the first 150 years},
   JOURNAL = {Bull. Amer. Math. Soc. (N.S.)},
  FJOURNAL = {American Mathematical Society. Bulletin. New Series},
    VOLUME = {6},
      YEAR = {1982},
    NUMBER = {1},
     PAGES = {9--24},
      ISSN = {0273-0979},
   MRCLASS = {57N10 (01A55 01A60 20H10 22E40)},
  MRNUMBER = {634431},
MRREVIEWER = {H. S. M. Coxeter},
       DOI = {10.1090/S0273-0979-1982-14958-8},
       URL = {https://doi.org/10.1090/S0273-0979-1982-14958-8},
}

@article {dupontsah,
    AUTHOR = {Dupont, Johan L. and Sah, Chih Han},
     TITLE = {Scissors congruences. {II}},
   JOURNAL = {J. Pure Appl. Algebra},
  FJOURNAL = {Journal of Pure and Applied Algebra},
    VOLUME = {25},
      YEAR = {1982},
    NUMBER = {2},
     PAGES = {159--195},
      ISSN = {0022-4049},
   MRCLASS = {53C40 (51M10 51M20 52A40 53A35)},
  MRNUMBER = {662760},
MRREVIEWER = {O. V. Shvartsman},
       DOI = {10.1016/0022-4049(82)90035-4},
       URL = {https://doi.org/10.1016/0022-4049(82)90035-4},
}

@article {morley:trisectors,
    AUTHOR = {Morley, F.},
     TITLE = {Extensions of {C}lifford's {C}hain-{T}heorem},
   JOURNAL = {Amer. J. Math.},
  FJOURNAL = {American Journal of Mathematics},
    VOLUME = {51},
      YEAR = {1929},
    NUMBER = {3},
     PAGES = {465--472},
      ISSN = {0002-9327},
   MRCLASS = {DML},
  MRNUMBER = {1506728},
       DOI = {10.2307/2370734},
       URL = {https://doi.org/10.2307/2370734},
}

@misc{braude:morley,
        author={Braude, Eric J.},
        title={Generalizing the {M}orley trisector and various theorems with realizability computations},
        year={2016},
        eprint={arXiv:1603.03463 [cs.CG]},
        note={\url{https://arxiv.org/abs/1603.03463}}
}

@book{schwartz:surfaces,
author="Richard Evan Schwartz",
title="Mostly {S}urfaces",
publisher="Amer. Math. Soc.",
year="2011"
}

@misc{gi:mpls,
author="John H. Conway and Peter G. Doyle and Jane Gilman and William P. Thurston",
title="Geometry and the {I}magination in {M}inneapolis",
year="1991",
eprint="arXiv:1804.03055 [math.DG]",
note={\url{https://arxiv.org/abs/1804.03055}}
}

